AGIR: Automating Cyber Threat Intelligence Reporting with Natural Language Generation

Cyber Threat Intelligence (CTI) reporting is pivotal in contemporary risk management strategies. As the volume of CTI reports continues to surge, the demand for automated tools to streamline report generation becomes increasingly apparent. While Natural Language Processing techniques have shown potential in handling text data, they often struggle to address the complexity of diverse data sources and their intricate interrelationships. Moreover, established paradigms like STIX have emerged as de facto standards within the CTI community, emphasizing the formal categorization of entities and relations to facilitate consistent data sharing. In this paper, we introduce AGIR (Automatic Generation of Intelligence Reports), a transformative Natural Language Generation tool specifically designed to address the pressing challenges in the realm of CTI reporting. AGIR's primary objective is to empower security analysts by automating the labor-intensive task of generating comprehensive intelligence reports from formal representations of entity graphs. AGIR utilizes a two-stage pipeline by combining the advantages of template-based approaches and the capabilities of Large Language Models such as ChatGPT. We evaluate AGIR's report generation capabilities both quantitatively and qualitatively. The generated reports accurately convey information expressed through formal language, achieving a high recall value (0.99) without introducing hallucination. Furthermore, we compare the fluency and utility of the reports with state-of-the-art approaches, showing how AGIR achieves higher scores in terms of Syntactic Log-Odds Ratio (SLOR) and through questionnaires. By using our tool, we estimate that the report writing time is reduced by more than 40%, therefore streamlining the CTI production of any organization and contributing to the automation of several CTI tasks.

==> Tables/02-STIX.tex <==
\begin{table}[!htpb]
    \caption{STIX entities and their description.}
    \begin{center}\resizebox{\columnwidth}{!}{
        \begin{tabular}{|l|l|}
            \hline
            \textbf{Entity Type} & \textbf{Description} \\ \hline
            Attack Pattern & A type of TTP describing ways adversaries attempt to compromise\\& targets.\\ \hline
            Campaign & A grouping of adversarial behaviours that describes a set of\\& malicious activities or attacks (sometimes called waves) that occur over\\& a period of time against a specific set of targets.\\ \hline 
            Course of Action & An action taken either to prevent an attack or to respond to\\& an attack that is in progress.\\ \hline
            Grouping & Represent a set of data that, in time, given sufficient analysis,\\& would mature to convey an incident or threat report.\\ \hline
            Identity & Represents actual individuals, organizations, or groups as well as\\&  classes of individuals, organizations, systems or groups.\\ \hline
            Indicator & Contains a pattern that can be used to detect suspicious or\\& malicious cyber activity.\\ \hline
            Infrastructure & Represents a type of TTP and describes any systems, software\\& services and any associated physical or virtual resources intended\\& to support some purpose. \\ \hline
            Intrusion Set & A grouped set of adversarial behaviours and resources with common \\& properties that is believed to be orchestrated by a single organization.\\ \hline
            Location & A Location represents a geographic location.\\ \hline
            Malware & A type of TTP that represents malicious code. \\ \hline
            Malware Analysis & Captures the metadata and results of a particular static or dynamic \\&analysis performed on a malware instance or family.\\ \hline
            Note & Informative text to provide further context. \\ \hline
            Observed Data & Conveys information about cyber security related entities such as files, \\&systems, and networks using the STIX Cyber-observable Objects (SCOs).\\ \hline
            Opinion & An assessment of the correctness of the information in a STIX Object\\& produced by a different entity. \\ \hline
            Report & Collections of threat intelligence focused on one or more topics.\\ \hline
            Threat Actor & Actual individuals, groups, or organizations believed to be operating\\& with malicious intent.\\ \hline
            Tool & Legitimate software that can be used by threat actors to perform attacks.\\ \hline
            Vulnerability & A weakness that can be exploited to negatively impact a system.\\ 
            \hline
        \end{tabular}}
    \end{center}
    \label{tab:stix}
\end{table}
